Is a Seat at the Table Enough? Engaging Teachers and Students in Dataset Specification for ML in Education

Despite the promises of ML in education, its adoption in the classroom has surfaced numerous issues regarding fairness, accountability, and transparency, as well as concerns about data privacy and student consent. A root cause of these issues is the lack of understanding of the complex dynamics of education, including teacher-student interactions, collaborative learning, and classroom environment. To overcome these challenges and fully utilize the potential of ML in education, software practitioners need to work closely with educators and students to fully understand the context of the data (the backbone of ML applications) and collaboratively define the ML data specifications. To gain a deeper understanding of such a collaborative process, we conduct ten co-design sessions with ML software practitioners, educators, and students. In the sessions, teachers and students work with ML engineers, UX designers, and legal practitioners to define dataset characteristics for a given ML application. We find that stakeholders contextualize data based on their domain and procedural knowledge, proactively design data requirements to mitigate downstream harms and data reliability concerns, and exhibit role-based collaborative strategies and contribution patterns. Further, we find that beyond a seat at the table, meaningful stakeholder participation in ML requires structured supports: defined processes for continuous iteration and co-evaluation, shared contextual data quality standards, and information scaffolds for both technical and non-technical stakeholders to traverse expertise boundaries.

==> scratch.tex <==
%\hari{I started reading the draft, left a few comments but I think the big thing is the findings need a bit of reorganizing to bring out the novel/interesting insight. I am thinking (1) Something along the lines of \hl{Contextualizing/aligning upstream tasks} with downstream use ( it’s not only about contextualizing data, but also contextualizing ML process decisions such as generalizability, collection process etc. )}

%\hari{check out figure 1 in this paper: \url{https://www.microsoft.com/en-us/research/uploads/prod/2019/03/amershi-icse-2019_Software_Engineering_for_Machine_Learning.pdf}}


%\hari{if you overlay context findings from our study on this pipeline you will see that teachers provide inputs in not just contextualizing the data but predicting consequences of data collection and modeling decisions in downstream use}

%\hari{\hl{ (2) Expertise and Collaboration }-- this can include insights about acknowledging different expertise, common grounding, translation, negotiating tradeoffs, challenges in reaching consensus on specifications}

%\hari{(3) \hl{Shifting Roles, Identities, and Support Needs} --- discuss interplay between different roles, identity crisis and overreliance on ML, and instances in which participants need scaffolds (knowledge scaffolding, design scaffolding, etc.)}

%\hari{currently atleast the initial findings reads a lot like the leaky abstractions paper  (organized by various knowledge blindness)we want to bring those concepts back in the discussion but not organize the findings in the same way}



Despite the \textit{linearity} of the ML data pipeline, participants approached specifications for each component by considering its interactions with other stages in the data lifecycle. While current definitions of stages (or steps) in the ML data pipeline are meaningful to engineering tasks, cross-discipline negotiation of concerns transcended discrete ML data tasks to contextualize designs. 



Across all sessions, domain experts contextualized upstream ML data tasks by considering downstream application context and hypothesized the consequences of collection and modeling decisions in downstream usage. By engaging diverse stakeholders in designing data needs in each stage of the pipeline, we find that collaborative practices disrupt the backward-looking engineering process of retroactively improving models when performance, utility, or ethical issues are surfaced. We observed stakeholders proactively anticipating challenges, considering trade-offs, recognizing data unknowns, and addressing bias and reliability threats.



RESULTS------------------

\section{Findings}
In each workshop session, we provided a diverse group of stakeholders with a specific application of ML in the education domain. We asked them to co-design specifications for each stage of the ML data pipeline. Teams engaged in rich discussions to define dataset composition, collection and labeling procedures, and evaluation metrics. By engaging in generative design thinking, participants shared domain expertise and personal (experiential) perspectives to anticipate challenges and navigate ethical considerations for data subjects and end-users. Across all sessions, knowledge sharing and constant co-evaluation facilitated the conceptualization of a human-centered ML data pipeline from the ground up. We summarize our study findings in terms of (1) contextualizing upstream tasks with downstream use, (2) collaboration strategies across expertise boundaries, and (3) shifting roles, identities, and support needs.

\subsection{Contextualizing Upstream ML Tasks within Downstream Use}
Typical ML data pipelines are linear and comprised of distinct data and modeling tasks. Our protocol based on current data documentation templates also followed a linear organization (see Fig ~\ref{fig:pipeline}). However, we observed that participants tended to approach specifications for each component by considering its \textit{interactions} with other stages in the data lifecycle. While current stages in the ML data pipeline are meaningful to engineering tasks, cross-discipline negotiation of concerns transcended discrete steps in the ML data pipeline. Across all sessions, domain experts contextualized upstream ML data tasks by considering downstream application context and hypothesized the consequences of collection and modeling decisions in downstream usage.  In engaging diverse stakeholders in designing data needs in each stage of the pipeline, we find that collaborative practices can disrupt the backward-looking engineering process of retroactively improving models when performance, utility, or ethical issues surface. Here we present observations about how stakeholders \textit{proactively} anticipate challenges, consider trade-offs, recognize data unknowns, and address bias and reliability threats.

  \begin{figure}[h]
\includegraphics[scale=0.25]{pipeline.png}
\caption{Major stages of the data lifecycle addressed in our workshops. The feedback arrows indicate the interactions between stages considered by participants to contextualize decision-making. %\hari{I like this figure, but should it come later in the paper? The arrows seem more like observational insights from the study. }
}
\label{fig:pipeline}
\end{figure}

\subsubsection{Domain Insights Shape Dataset Specifications}
Across all sessions, participants initially approached design in the composition stage with high-level requirements (ie, student photos, academic transcripts, resumes, written work, etc.), targeting a general purpose application with broadly defined adoption contexts. However, as groups continued to engage in co-design, teachers supported teams in refining specifications in ways that captured  the nuances of realistic downstream needs.  


they generated specifications with a rich set of context-based features that captured the nuances of realistic downstream needs. By sharing rich anecdotal insights and examples, teachers (i.e., domain experts) introduced \textbf{contextual variables} that prompted the group to rethink the scope and generalizability of dataset composition. For example, teachers noted the effect that student age, educational institution type, teacher experience level, and community socioeconomic status may have on predicted outcomes, motivating the group to decide between expanding data representation requirements to support generalizability or limiting the scope of the application to maintain accuracy. Guided by classroom experience, teachers in all sessions advocated for an applied understanding of representation, contributing important features of educational environments to augment familiar demographic variables. While normative data practices associate diversity and demographics with a limited set of attributes, teachers highlighted the richness of what diversity means in education.
%\hari{Again elaborate, we all assume diversity and demographics mean certain attributes. Teachers highlighted the complexity and richness of what diversity means in education}. 
Beyond age, gender, and race, significant student attributes are grounded in the complexity of diverse learning contexts. Teacher T2 explained:
\begin{displayquote}
T2 (Student Engagement Image Classification): “Diversity can mean so many different things beyond just physical attributes. It’s like diversity of environment, what they're working on, because focusing on math might look different than focusing on reading or art, … or if they're working with other people, … but those are things that could play into a student's engagement level.”
\end{displayquote}

Across workshops and design scenarios, specifications for subgroup representation involved data regarding educational environments, including school type, urbanicity, teaching quality and subject matter, and teacher and parent demographic attributes. The range of encoded information contextualizing diversity stands in contrast to common engineering interpretations of representation standards. Domain experts additionally introduced student-specific context variables known to significantly differentiate learning experiences and outcomes, including socio-economic status, language learner status, and first-generation or immigrant status. One contextual variable commonly raised by teachers involves the presence of learning differences or disabilities such that would require an individualized education program (IEP). Teacher T1 described:
\begin{displayquote}
T1 (Student Engagement Image Classification): “The other thing is maybe having data knowing whether a student has an IEP… if a student is diagnosed with ADHD they are not going to be as focused as the student without. There are also emotional learning disabilities… students who are having particular traumas at home … and these are actually pretty relevant in terms of motivation and engagement.”
\end{displayquote}

The complexity of possible values for a large collection of contextual variables representing diverse learners and environments prompted participants to consider tradeoffs between the size of the dataset and scope of the application scenario. Concerns about the amount of data required to ensure equitable distribution of subgroups represented in the dataset, combined with concerns about prediction accuracy for underrepresented subgroups, led participants to consider whether the model should be designed to apply only to a specific age group, learner status, or type of school. In these discussions, engineers contextualized downstream modeling options and machine learning processes to support data composition and target application decisions. Engineer E6 explained the practice of comparing multiple models, in response to a disagreement between non-technical stakeholders regarding semantic differences in public and private school data:
\begin{displayquote}
E6 (Student Drop-out Risk Prediction): “In machine learning, it's pretty common to have multiple models… and it's called ensembling where you just put them all together… then choose the best results… but then you have… different understandings of the same data, and that can be pretty useful, especially if we want to compare.” 
\end{displayquote}
In most sessions, engineers shared expertise highlighting the affordances of machine learning, downstream opportunities to test multiple design choices, and tradeoffs in the accuracy and interpretability of technical methods. These technical contributions situate the design of dataset composition in  downstream processing and modeling applications, adding methodological context to the real-world factors shared by domain practitioners. 

\subsubsection{Mitigating Bias and Reliability Threats}
Participants incorporated the identification of future threats to data quality in the design of data collection specifications. By introducing evaluative considerations early in the data pipeline, groups contextualized data needs to preemptively mitigate bias and reliability risks. While designing data collection procedures, stakeholders leaned on student perspectives as data subjects to anticipate concerns with false, malformed, and missing data. Students shared their personal experiences with survey fatigue, inadequate incentive structures, and creating fake signals. Helping the group to maximize response rates for collecting student resumes, student S4 explained their reactions to various collection strategies:
\begin{displayquote}
S4 (Resume-based Career Recommendation): “As a student I’m probably not going to bother sending off my resume for no compensation, but compensate me and I might try and game it. However, if you do ask me for the resume with compensation and a survey, I feel like answering the survey questions is maybe going to invest me more than if I was just firing off PDFs.” 
\end{displayquote}
In several sessions, stakeholders grappled with the possible impacts of uncooperative data subjects and adjusted collection procedures to prevent unwanted outcomes. Their hypothesized solutions include information campaigns to improve data subject buy-in, designing non-invasive collection methods to avoid disrupting authentic student behaviors, and enforced completion of data fields in the survey instrument to avoid downstream handling of missing data. 
In the evaluation stage of the design protocol, the prevention of data quality threats further motivated stakeholders to design data cleaning procedures that detect and remove malformed or false data and standardize data fields. Regarding variability in the interpretation of grade labels in collected district writing samples, engineer E10 explained:
\begin{displayquote}
E10 (Automated Essay Grading): “Some of the schools are strict on grading, and some of them are not, so maybe we also need to align those... maybe we need to do the data engineering to make all of these standardized.”
\end{displayquote}
Across all sessions, groups designed data cleaning processes, including extracting features from raw data, reformatting data according to shared standards, and comparing data against baseline values. Data representativeness and appropriate distributions of diverse subgroups emerged as a recurrent theme regarding data quality in the evaluation stage. Participants designed processes to pursue this standard by returning to the design of collection procedures and augmenting data from underrepresented groups via additional collection processes, extrapolation, or borrowing data from other contexts. 
Another major component of mitigating bias is the specification of labeling procedures. A common strategy observed across sessions involved validating labels through multiple sources and ensuring intercoder reliability. Considering the authenticity of labelers, and drawing upon their previous experience as a special-education teacher, designer D2 suggested engaging data subjects in self-identifying labels:
\begin{displayquote}
D2 (Student Engagement Image Classification): “I think it would be really important actually to have students self identify. The people who are interpreting that facial expression are going to have a different interpretation than the person that made it. But like having the comparison between the students' self reflection and the teachers' perception and measuring that gap in between.”
\end{displayquote}
For sessions in which groups decided to repurpose an existing dataset rather than collecting raw data, participants expressed skepticism over potentially biased labels and concern for the downstream effects of mislabeled examples. Participants committed to hiring multiple labelers and calculating agreement scores, auditing labels in second-hand datasets, and specifying requirements for the qualifications and diversity of labelers as a precaution for obtaining reliable labels. While labeling procedures are discussed in the collection stage of the workshop protocol, participants often discussed data quality standards and data evaluation concepts to anchor their design decisions.
Finally, though participants were tasked to consider bias mitigation in the collection stage of the protocol, groups conceptualized bias beyond that inherent to the composition of a dataset. Groups noted the importance of transparency of data processes to mitigate applied bias in downstream use cases. In the automatic essay grading scenario, all groups considered reusing second-hand data from a standardized testing service, while observing that work samples from students financially able to access the service were over-represented. Specifying the communication of the biases that cannot be mitigated, teacher T8 described:
\begin{displayquote}
T8 (Automated Essay Grading): “I think also just naming the biases that you cannot reduce, or that you cannot address, so if you’re using a certain set of criteria that’s constructed by the AP, the emphasis on language conventions is. . . biased towards standardized academic English. Okay, if we can’t eliminate this bias, we can at least name it in our process.”
\end{displayquote}

\subsubsection{Anticipating End User Experiences}
We observed a recurring focus on downstream end-user experiences to contextualize collection and evaluation procedures. Rather than leaning on technical language and conventional engineering metrics for model performance in the evaluation stage of the protocol, domain experts encouraged groups to prioritize evaluation of the application as a whole. Adding to the conversation about testing procedures validating the accuracy of the model, teacher T9 advocated for the most relevant domain-specific performance metric in education:
\begin{displayquote}
T9 (Automated Essay Grading): “The quality should be measured by the learning outcomes of the students… like how they're responding to the feedback that they get from the tool. I know that's really hard.”
\end{displayquote}
Across all sessions, groups acknowledged the tradition of standardized quantitative metrics and their inability to capture the real-world effects of a machine learning application. Despite recognizing the incompleteness of existing metrics, participants faced difficulties creating new ones that better serve contextual needs.  The challenge of designing evaluation specifications prompted stakeholders to revisit decisions in earlier stages of the data pipeline, often returning to design decisions in the data collection stage and selecting different labels that would better support end-user goals.
Beyond a single metric, participants conceptualized the evaluation stage as ongoing procedures to be observed as models are deployed to real-world applications. Groups anticipated the need for monitoring application behavior and efficacy iteratively over time. Engineer E3 explained:
\begin{displayquote}
E3 (Student Engagement Image Classification): “You would also need a feedback loop. How do we know whether people are satisfied with it or not?” 
\end{displayquote}
While utility and satisfying end-user requirements represent one evaluative standard, other groups expressed concern about model effectiveness over time as students learned to “game the system”. Participants designed continuous random evaluation procedures on application data, suggesting human-led audits of a percentage of predictions, and regularly updating the model with feedback.

By moving freely along the data pipeline, participants situated data needs and machine learning processes in domain-aware contexts, anticipating end-user experiences and proactively mitigating threats to data quality. The separation of concerns between data, modeling, and application work represents an engineering-centric framework. We find that multi-stakeholder groups engage in decision-making holistically, contextualizing data specification with use case elicitation and trade-offs in every stage of application development. 


\subsection{Collaboration strategies across expertise boundaries}
While role-based knowledge boundaries have traditionally limited opportunities for collaboration between machine learning engineers and domain experts, we observed multi-stakeholder groups engaged in boundary-spanning collaborative practices. Participants employed expertise-specific strategies to overcome knowledge gaps and build cross-discipline understanding. Through practices of translation and advocacy, groups amplified diverse perspectives, built common ground, and navigated ambiguity.
\subsubsection{Translation}
Non-technical stakeholders often perceive barriers to participation in technical decision-making due to knowledge gaps in machine learning capabilities and processes. Acknowledging the lack of familiarity with ML in the education domain, teacher T9 explained:
\begin{displayquote}
T9 (Automated Essay Grading):  if you were to go into a classroom, I think the majority of high school teachers in the United States. . . if you say machine learning and natural language processing and algorithms, they have no idea what you’re talking about. That’s not because they’re stupid, it’s just because it’s a very niche topic that you don’t really hear much about when you’re in the classroom. There needs to be some sort of middle ground.. of translation to lay folks that don’t live in this world of zero and ones.”
\end{displayquote}
While jointly negotiating data needs, engineers across all sessions engaged in the collaborative practice of translation. Through translation, technical experts went beyond merely reframing practitioner priorities into machine learning terms in data specifications, but actively shared technical knowledge to establish common ground and scaffold practical understanding for domain expert participation in co-design. One mode of translating contextual data needs into technical specifications involves evaluating the feasibility of teacher requests. In the data composition stage, when teacher T5 advocated for augmenting standardized exam scores with local classroom performance metrics, engineer E5 considered the feature in terms of its technical representation:
\begin{displayquote}
T5 (Student Drop-out Risk Prediction): “Would it be much harder to add in that layer? It’s just whether they have passed a class with a certain letter, in this case it’s a C or higher.”
\end{displayquote}
\begin{displayquote}
E5 (Student Drop-out Risk Prediction): “I wouldn’t say it's a hard feature to add, it sounds like a binary feature. It’s a yes or no, right? You add a column, and the value is yes or no. Yeah, I think that’s feasible.”
\end{displayquote}
We observed engineers across all sessions applying their technical knowledge to support teacher feature requests whenever feasible. Translation occurred in the encoding of teacher-raised relevant data fields, as well as the planning of technical processes in the data collection and evaluation stages to accommodate use case concerns. We observed engineers engaged in translation by clarifying machine learning processes to support broader practitioner concerns and values. For example, given the publicity surrounding privacy violations and biases along demographic dimensions in machine learning, nontechnical stakeholders displayed a sensitivity to collecting race, age, and gender variables. Addressing confusion and unease about the collection and use of demographic data, engineer E2 explained:
\begin{displayquote}
E2 (Student Engagement Image Classification): “You can decide to use [demographic variables] to understand your data, and then… you already know the data is potentially biased. So when you build your model, you keep that in mind, and you refine your model to cope with that bias.”
\end{displayquote}
By translating domain priorities into evaluative specifications, the engineer reached across knowledge boundaries and deepened collective understanding of the use of demographic data in machine learning processes. As a practice, translating allowed engineers to use their technical expertise to amplify the voices of practitioners, enabling non-technical stakeholders to contribute to the construction of human-centered data needs. Using the shared scenario context, engineers explained trade-offs in data and modeling choices, building the technical foundation to support domain expert participation. While considering representation of diverse school settings in the data composition stage, engineer E6 described their considerations in specifying the scope of a model:
\begin{displayquote}
E6 (Student Drop-out Risk Prediction): “If you train this model for just this one school, then you would be looking at all of the previous data that you have from that school… with the downside being that you might not have enough data… for the model to learn from, or it might draw the wrong conclusions. One of the benefits of training a model… on all the schools in the district… is that you have a lot more data points. But the downside of that is like maybe you're at a really poor school, and all the other schools in your district are really rich, so the drop-out patterns might be different.”
\end{displayquote}
\begin{displayquote}
T6 (Student Drop-out Risk Prediction): “They both seem to have downsides, but maybe per-district is better, because if it's generalized for everyone… then the inaccuracy is higher, but… there's a lot more data, so it's better to be more accurate.”
\end{displayquote}
By leaning on the design scenario, the engineer contextualized the effects of technical decisions in domain-relevant terms, enabling the teacher to engage in the evaluation of the trade-off. While technical terms such as “accuracy” and “generalization” had been used previously in the workshop, they had not been taken up by the teacher. By translating the contextual costs and benefits of modeling choices, the engineer empowered the teacher to then take up technical language and contribute to decision-making.
In many sessions, the technical stakeholders took additional care to educate non-technical stakeholders regarding technical details through extended dialogue, actively scaffolding their uptake of technical language in the design process. In a few sessions, engineers employed metaphors and likened ML to familiar analog processes, tailoring technical knowledge in their explanations to serve as a broker between domains. We also observed that translation is practiced predominantly by technical experts. Due to the the social nature of the education domain, technical experts may more easily make assumptions about educational contexts without requiring translation from domain experts, while the infusion of technology in education is a recent and disruptive change foreign to many domain practitioners.

\subsubsection{Advocacy}
The high-stakes nature of the educational field necessitates developing machine
learning applications prioritizing practitioner experiences. In the collaborative context, domain experts engaged in advocacy, leaning into extended discourse and emotion-driven language, urging out-of-domain stakeholders to confront the complexities of education systems and hidden implications of data decisions. As student S4 described, \textit{“you have to try and be an advocate, and if you're going to deploy a system like this you're going to have to come up against people who do advocate for other interests”}. Indeed, teachers and students across sessions characterized their collaborative participation as advocacy. They advocated for fairness and utility priorities motivated by their domain contexts and lived experiences while negotiating cross-cutting requirements. 

By surfacing critical downstream implications of data labels, feature encoding and modeling choices, teachers voiced values and sensitivities central to the education space. Teacher T6 warned against possible downstream harms due to the language of default labels in the student drop-out prediction scenario (e.g., "dropped out" and "did not drop out"):
\begin{displayquote}
T6 (Student Drop-out Risk Prediction): “Then these students will be labeled like dropouts, and then it gives administrators a reason to push students like this out of school.”
\end{displayquote}
Teacher T6 instead advocated for student-centric labels, reframing the application scenario to predict whether a student was "on track to graduate". The complex structure of educational systems produce role-based differences in interests, priorities, and interpretations of model results. While school and district administrators value drop-out metrics, teachers prefer a reversed framing featuring student progress towards positive goals, aware of the real-world implications for how students flagged by the system may be treated. By explaining their experience-motivated understanding of mentalities and practices in the downstream application context, teachers in several sessions advocated for data specifications that avoid that perpetuation of system inequalities.

Similarly, in automated essay grading scenarios, teachers argued against training a model to predict standalone evaluative scores, and preferred the growth-based framing of providing targeted feedback directly to students. Across all sessions focusing on this scenario, teachers advocated for the increased fairness and utility of using labels that identify features of student writing. In engagement classification scenarios, several teachers expressed concern at the use of “distracted” and other negative labels. Domain experts advocated for positively-framed labels to inform instructional choices, citing the potential downstream effect of teachers unfairly developing negative attitudes toward negatively labeled students. 

In many cases, groups ultimately adopted the teacher-recommended labels, indicating an openness to identify with practitioner values of supporting student autonomy and avoiding punitive administrative repercussions. However, teachers occasionally received extensive push-back from technical stakeholders. In these cases, teachers persisted in their advocacy until groups understood the intent and gravitas behind their concerns. In one session working with the engagement classification scenario, the teacher and engineer engaged in an extended heated exchange regarding the ethics of classifying students with emotion-based labels. Teacher T3 explained the racialized underpinnings of assuming the emotional states of students in classroom practice:
\begin{displayquote}
T3 (Student Engagement Image Classification): “I would personally feel like that's something I can decide based on myself and my rapport with the students. If a student… was frustrated or confused, to use those labels, I would be concerned about… stereotyping. It’s a really big problem in education, how black students versus white students, how their behaviors read to a lot of white teachers as different, even though it can just be their specific cultural background.”
\end{displayquote}
While advocating against using labels that make assumptions about the emotional states of students, teacher T3 alludes to two other sensitive themes in the education domain: the historical context of racially biased perceptions of student behavior, as well as ML's infringement on the teacher’s role of human judgment in the classroom. The exchange emphasized the weight of these critical tensions in education and the prominence of racial and cultural considerations to the domain. A similarly heated discussion in another session involved the collection of teaching quality evaluation data for predicting student drop-out risk. Teacher T5 argued that the use of teacher evaluation data by administrators would impact teacher unions and staffing policies, further complicating an existing district struggle with protections for teachers. By contextualizing the social and political constructs connected to technically objective variables, teacher advocacy enabled groups to collectively situate data decisions in a complex ecosystem and approach designs with respect and sensitivity toward the worldviews encapsulated.

Across many sessions, advocacy operated through the sharing of personal lived experiences. While designing dataset composition in the automated essay grading scenario, teacher T9 argued against relying on quantified rule-based grammatical features to evaluate student writing:
\begin{displayquote}
T9 (Automated Essay Grading): “When I taught English on the west side of Chicago, ninety-nine percent of my students were African American. I understood what they were saying, but it was not written sort of like traditional academic American English. You don't want to penalize the student for the culture that they live in, and the language that they speak.”
\end{displayquote}
Teacher T9 reflected on their personal struggle to both respect individual student backgrounds and prepare students for future strict evaluative environments, and admitted that they still feel uncertain about the balance. The problem-solving nature of the co-design sessions invited sensitive practitioner stories involving difficulties faced in the classroom. Despite the relative vulnerability required of teachers and students compared to other roles, they met the task and eagerly advocated for the complex realities in the domain. 

\subsubsection{Ambiguity}
During time-limited co-design sessions, participants navigated the balance between big picture discussions and specifying design details. Engaging in high-level discussions required stakeholders to develop a sense of comfort with ambiguity, accepting data unknowns and unfinished design decisions. Though participants expressed uneasiness about ambiguity in the design task, engineer E5 noted how the process stands in contrast to designing with a false sense of certainty:
\begin{displayquote}
E5 (Student Drop-out Risk Prediction): “When we’re talking about designing a system everybody wants to pretend they know more than they think. When we talk about making a decision everybody feels like they already know the answer, like they should know the answer. In this kind of setup. . . I feel that it’s okay for me to not know the answer. . . and I rely on other roles.”
\end{displayquote}
The presence of diverse stakeholders facilitates a collective acceptance of ambiguity while choosing proactive big picture data planning. Engineers in other sessions echoed their ultimate appreciation of the open-ended nature of design decisions, given the relative infrequency of higher level conversations in typical machine learning processes.


\subsection{Shifting Roles, Identities, and Support Needs}
Our study surfaces role-based collaborative dynamics and persistent knowledge gaps and boundaries that complicate contribution in multi-stakeholder settings. Although participants engaged productively in the co-design process, we observed groups making assumptions, building on misconceptions, and getting stumped by shared unknowns. Stakeholders struggled with role-based identities and contributions. We identify challenges and support needs for engaging diversestakeholders collaborative data specification.
\subsubsection{Rigid responsibility boundaries}
While co-design sessions encouraged many boundary-spanning practices between engineers and domain experts, some role-based boundaries persisted and hindered collaboration. Several engineers maintained a bounded view of responsibilities and liability in data decisions. Especially for evaluations of ethical decisions, fairness for demographic subgroups, and consent practices, engineers were quick to delegate to specialized entities. Regarding the representation of subgroups in the composition stage of the protocol, engineer E1 explained:
\begin{displayquote}
E1 (Student Engagement Image Classification): “This is usually something that you shouldn’t be asking just anybody. I’d leave this question up to the ethics review panel professionals.”
\end{displayquote}
In an industry made efficient through role-based specialization, engineering responsibilities may be narrowly defined. Ethical standards are often handled by designated professionals in teams separate from engineering processes. Beyond preferring a separation of concerns, engineers indicated being accustomed to a standard industry practice removed from dataset designs choices. In the automated essay grading scenario, engineer E10 explained their unease in the data collection stage of the protocol, while deciding between several ideas for labeling schemes:
\begin{displayquote}
E10 (Automated Essay Grading): “We don’t usually have that many options. You don’t have a choice, we really work with what we have. I don’t design how people give their data.”
\end{displayquote}

While engineers engaged in knowledge sharing and translating practices, some did so to varying degrees of effectiveness. Despite an engineering effort to break down technical barriers, some teachers continued to feel intimidated by tech blindness. Others further struggled to contribute when additionally perceiving a misalignment between the student age group they had experience teaching and the target student age group for the machine learning application. Teacher T4 explained:
\begin{displayquote}
T4 (Resume-base Career Recommendation): “I didn’t think I had as much to add from an education perspective because my background is with a lot younger students.”
\end{displayquote}
Despite differences in the age group or subject matter in which teachers are more experienced, teachers nonetheless contribute domain expertise. By underselling their understanding of context from working in the education system as an educator more generally, some teachers viewed their own stakeholder role as a direct end-user rather than co-designer. In several sessions, teachers fell more silent to self-imposed boundaries and misconceptions of qualifications for participation.
\subsubsection{Persistent knowledge gaps}
Groups face knowledge gaps regarding the identification of data owners. Despite the collection of educational data from academic records, classroom observations and student work, teachers were unsure of data ownership regulations. Referring to collecting student essay data, teacher T8 explained:
\begin{displayquote}
T8 (Automated Essay Grading): “They probably live in the teachers’ district or school Google Drive, or whatever they’re using. . . and so I’m not really sure who owns the rights to those.”
\end{displayquote}
Data ownership is further complicated by the storage of data through edtech systems with opaque data privacy terms negotiated with school administration. Even for data assumed to be maintained directly by school administration, teachers could not identify ownership and access processes. With regard to obtaining student academic records, multiple teachers expressed the need for school administrators to be present. Circumstances in education systems introduce variance in roles and responsibilities across districts, complicating the task of bringing stakeholder voices to the table. For domain experts, this knowledge gap may point to an unknown stakeholder and data owner in school administration who should be engaged in designing data specifications.
Engineers similarly make assumptions about data availability. Regarding a variety of student academic and financial records, engineer E6 assumed:
\begin{displayquote}
E6 (Student Drop-out Risk Prediction): “A lot of this data can be directly collected through the College Application, right? Sounds like a safe bet to say the university has all of them, I mean they keep a record of everything. It’s probably already marked in their system.”
\end{displayquote}
For engineers, these assumptions may be reflective of their training, in which datasets are given rather than constructed. Despite unknowns regarding data use agreements, shape and composition of data, and the right data owner to contact, engineers maintained confidence that data exists.

Despite involving stakeholders advocating for the legality of data privacy issues, knowledge gaps persist in data security and access. Engineer E1 used an assumption of security to justify haphazard consent practices:
\begin{displayquote}
E1: “For educational applications where there's going to be very little chance of any kind of deleterious impact or data leak, … you can ask the children to check a box saying my parents approve.”
\end{displayquote}
Both technical and non-technical participants expressed relaxed attitudes toward data security, citing a lack of incentive for malicious data breaches. Teacher T2 explained, \textit{“I don’t see why anybody would even want to hack into something that the schools were using.”}

\subsubsection{Shifting stakeholder identities}
While the teacher, engineer, and legal professional held clear participatory roles with established expectations for contribution, the collaborative identities of the student and UX professional roles were less defined. Student S4 explained, “consistently occupying the student perspective... is difficult because the students are not going to be involved in every stage.” Lacking a defined structure of contribution and being the youngest in a group of professionals, students often removed themselves from their primary role of end-user and contributed to the collective task in a general co-designer capacity. Students eagerly participated in technical co-design, offering data collection and modeling ideas unrelated to the student perspective. While the group discussed potential features to include in the dataset composition stage of the protocol for the student drop-out prediction scenario, student S5 explained their ideas for unconventional survey methods:
\begin{displayquote}
S5 (Student Drop-out Risk Prediction): “Oh, it might be interesting to have students survey each other almost, and. . . this feels kind of creepy, but assigning. . . one person in each of your classes and then say ‘does this person seem okay or do they seem like they’re gonna fail out of school’, I think that that could be interesting.”\\
E5 (Student Drop-out Risk Prediction): “I could see the potential bullying material for that.”
\end{displayquote}
In an effort to contribute to the design task, the student had lost empathy with data subjects, requiring the engineer to point out the potential downstream harms. Several students in the student drop-out prediction scenario additionally advocated for collecting mental health and other sensitive information from students. Across all sessions, students often referred to data subjects as “they” and separate from themselves. 

We find that, across all sessions, stakeholders lean on prior roles and experiences, often demonstrating multiple competencies, and shifting between these identities throughout the collaborative co-design process. Several legal professionals additionally had technical experience such that they could contribute ML best practices and participate in translation practices. Several designers and engineers had prior experience in various positions in the education sector such that they could contribute ideas motivated by domain expertise to contextualize data. Every stakeholder either remembers the experience of having been a student or is closely connected with a student through their social relationships, such that they could speak on behalf of student interests. Meanwhile, students struggled to always contribute through the role of a data subject and end-user, and instead often opted to participate through the role of a co-designer of data specifications.

UX professionals similarly lacked definition in their participatory roles. In the debriefing of the workshop, engineer E7 reflected, \textit{“this problem didn’t have too much to do with the UX perspective, so the collaborators have unequal representation in the discussion.”} By organizing co-design workshops that engage diverse stakeholders, the setting of the research study performed some of the traditional roles of designers, confusing the group understanding of their expected contribution. Across sessions, several designers additionally maintained a role-based separation of concerns, limiting their contribution to technical topics. Removed from technical contribution and lacking the personal domain experiences of teachers and students, designers often faded into the background. 


INTRO ------------------

% School districts increasingly and controversially require students to use school-provided technology that tracks every sentence students write and every website students visit, whether from school or at home.' In recent years, algorithms have become applied in educational practices at scale for a range of applications, often high-stakes, including dropout prediction (Christie et al., 2019; Milliron et al., 2014), automated essay scoring (Ramineni & Williamson, 2013), graduate admissions (Waters & Miikkulainen, 2014), and knowledge inference (Ritter et al., 2016)


% As indicated earlier, our goal was to understand (1) what knowledge diverse experts bring to specify ML data needs from the ground up, (2) what assumptions and biases they hold in ascribing those requirements, and (3) whether and how they communicate and align social and technical perspectives around AI in education


The rapid development of machine learning (ML) applications in education has raised issues of fairness, accountability, transparency, and utility in their implications for practitioners and vulnerable student populations \cite{baker2022algorithmic, perrotta2020deep, pedro2019artificial}. Despite the promise of ML to facilitate learning processes with intelligent tools, ethical intentions are not by themselves sufficient \cite{holmes2022ethics, reich2017good}. The extensive adoption of ML applications in administration, instruction, and learning has been met with emerging ethical harms, including systematic inequalities in recommender systems \cite{marras2022equality} and high-stakes automated decision-making \cite{aied_chapter}, surveillance and civil rights concerns in facial recognition systems \cite{whittaker2018ai}, data privacy concerns \cite{potgieter2020privacy, feathers-1, feathers-2} and disparities in student propensities to consent \cite{li2022disparities}. The intensifying problem space is complicated by the underlying challenges facing ML in education: undefined policy-level guidelines \cite{schiff2022education}, insufficient teacher education and involvement in ML development \cite{bogina2022educating, schiff2021out, roll2016evolution}, underdevelopment of inclusive and high-quality data systems \cite{Ocumpaugh2014, gardner2019evaluating}, and lack of ethical regulation and transparency in data collection, use, and dissemination \cite{pedro2019artificial}. 

One explanation behind unmet expectations of ML applications in education exists in the process tensions between engineering priorities and domain-specific practitioner needs. Traditional ML development processes undervalue the role of trustworthy training data and dataset accountability \cite{10.1145/3411764.3445518}. Despite the critical role of data in algorithmic predictions, training data is given inadequate consideration in current ML software workflows. Engineers often optimize the ML development process by defining data requirements -- including data types, features, labels, and the number of data points -- in an ad hoc manner. This approach falls short of capturing the needs of end-users and omits important contextual features of real-world data. While researchers have created guidelines for downstream data evaluation and documentation, standard practices remain undefined in upstream data specification.

Furthermore, traditional engineering processes limit engagement with domain experts and end-users \cite{10.1145/3491102.3517537}. When included, diverse experts only converge in ML development after crucial data-related decisions have been made. Addressing the disconnects between stakeholders in development practices requires early collaboration, active construction of common ground, and co-created scaffolds to transcend knowledge boundaries. 

As ML architectures stabilize, a recent methodological shift towards data-centric AI has re-prioritized the design of training data characteristics as the core mechanism to achieve desired performance. Data-centric methods present an opportunity to address fundamental data planning and collection issues by involving diverse stakeholders early in the ML development process.
\\
We ask the following research questions: 
\begin{itemize}
    \item What do diverse stakeholders bring to the table when engaging in the proactive co-design of data specifications?
    \item How can we systematically support and amplify diverse stakeholder voices in the ML data specification process?
\end{itemize}

To investigate these research questions, we conduct a series of structured workshops engaging experts and stakeholders across domains in the collaborative co-design of training data specification for ML applications in education. Workshops guided stakeholders through the process of collectively defining dataset characteristics, discussing representativeness and validation criteria, developing labels, and planning ethical data collection strategies for several application scenarios (e.g., student drop-out risk prediction, automated essay grading, student engagement image classification). Forty participants took part in our study, representing ML engineer, teacher, student, UX designer, and legal expert roles. By observing how different experts advocate for human-centered data, we identify proactive data specifications contextualizing upstream tasks in downstream use, collaborative strategies across expertise boundaries, and barriers to effective co-design.

This paper contributes to the emerging practice of data-centric AI, collaborative processes in human-centered AI, and the growing literature on practitioner needs regarding ML applications in education. We conclude by discussing the implications of our findings, including developing shared standards, information scaffolds, and supportive tooling to support multi-stakeholder contribution to ML data specification and assessment. Finally, we analyze the affordances and limitations of having a seat at the table and discuss directions for future research designing collaborative processes for engaging stakeholders in the education domain.

%\hari{What are our research questions? }


\section{Discussion}
Our findings demonstrate the vital role that multi-stakeholder collaborations play in the design of data specifications. Through conducting workshops anchored in the co-design of ML datasets in the high-stakes field of education, we highlight practitioner efforts to contextualize domain and procedural knowledge, establish common ground, and mitigate downstream harms. Participants engaged in a generative process of negotiating data requirements and quality in each stage of the data pipeline, placing due emphasis on the proactive design of human-centered systems. We emphasize the value of engaging domain experts and discuss the challenges facing the scalable implementation of the collaborative processes explored in this study. We characterize our contributions in terms of implications for the work of data specification and support needs for future integration of multi-stakeholder collaborative processes in responsible data use in education.  

\subsection{Is a seat at the table enough?}
Critical scholarship has explored the tension between developing machine learning systems for scalable production and involving end users in the design of these systems~\cite{sloane2020participation}. By establishing a structured co-design environment in which diverse stakeholders were given a seat at the table, many of our participants engaged in organic negotiations to overcome knowledge boundaries to establish common ground through collaborative strategies. We found that participants both made significant contributions to the specification of data requirements and faced challenges in the co-design process. In this section, we discuss the affordances and limitations of stakeholder involvement in our workshop sessions through two participation frameworks and the application context of the education domain.

Delgado et al. describe an analytical framework for the dimensions of participation, designed for practitioners to assess the extent to which a process for participation meaningfully empowers diverse stakeholders in the design of ML applications~\cite{delgado2021stakeholder}. Consultation, involvement, collaboration, and empowerment are scaled degrees of participation, assessed at five decision points addressing the motivation, stakes, attendance, form, and power distribution in participation processes. Sloane et al. caution against ``participation washing,'' in which the narrative of participation obscures power dynamics, and the extractive nature of collaboration~\cite{sloane2020participation}. By critically framing participatory design practices as work, consultation, and justice forms, practitioners may assess the authenticity of collaborative processes. Here we reflect on the nature of participation in our co-design sessions. 

\subsubsection{Affordances of co-design}
In formulating our workshop protocol, we propose a preliminary approach to multi-stakeholder co-design. Our findings 


Our workshop sessions represent an exploratory approach to multi-stakeholder co-design processes, and they effectively demonstrate the crucial role of collaborative data specifications. Teachers shared domain expertise impacting critical features in dataset design and model performance. Out-of-domain experts commonly expressed surprise while recognizing their own knowledge gaps and disrupted assumptions regarding contextual variables relevant to the education domain. When reflecting on their collaborative experiences, engineers across all sessions discussed the narrow technical focus of traditional ML development processes, admitting often misplaced efforts and overlooked practitioner priorities. The co-design of data specification is a participatory structure with stakes that empower stakeholders to contribute to the scope and purpose of ML applications. In these workshops, participation is motivated by better alignment between ML applications and stakeholder needs. While the rationale behind the workshop design is representative of a high degree of participation according to the dimensions of participation framework, the design falls short of empowering stakeholders due to a lack of accountability process. Without accountability for the quality of implementation of stakeholder contributions, participation workshops can become performative, failing to actualize the recommendations of diverse stakeholders.

Groups additionally realized the value of “big picture” conversations to anticipate future harms by incorporating a contextual understanding of how data choices affect end-users and their environments. Though our workshop protocol had been developed with the intention of stakeholders converging on design decisions in each stage, groups engaged in a process of ideation and filtration that often resulted in the recognition of multiple possibilities for further exploration. In line with collaborative approaches emphasizing the importance of friction and disagreement \cite{keshavarz2013design}, diverging perspectives encouraged participants to develop an appreciation for ambiguity. The construction of a jointly negotiated framing, in a participatory process in which diverse stakeholder expertise is valued equally, promotes a plurality of designs in the resulting specifications. In the process, participants admit unknowns and rely on the collective knowledge of those at the table.

\subsubsection{Unequal burdens}
To engage in effective co-design, participants traversed expertise-boundaries by practicing collaborative strategies unique to their roles. We observed domain experts striving to establish common ground by sharing vulnerable personal experiences and advocating for practitioner needs in a complicated historical and socio-cultural context. Because all participants have personally experienced education systems as students, out-of-domain stakeholders confidently make assumptions, leaving teachers and students with the emotional burden of advocating for their classroom experiences and navigating technology-centric pushback. In contrast, a heavy communicative burden is placed on the role of technical experts as boundary spanners. Because domain practitioners in education feel significant barriers to contributing to the design of highly technical applications, engineers must support the central role of translation in collaborative practice. In the most positive collaborative sessions, we observed engineers exhibit a willingness to teach foundational concepts and processes, patiently explaining technical tradeoffs. By translating domain-specific requirements to data and modeling requirements, engineers were able to address the needs advocated by non-technical domain experts. However, despite the productive ends of these collaborative strategies, they place extensive capacity demands in unique ways on both technical and nontechnical participants. Without structured support, multi-stakeholder collaboration is a high-lift endeavor. Across our sessions, groups recurrently fell back on engineer-led linear decision-making when any stakeholder lacked the skill, knowledge, or energy capacity to meet these collaborative requirements.

In Sloane et. al's framing of the forms of participation, the co-design workshops in this study align most closely with "participation as consultation", in which diverse stakeholders are engaged in various stages of episodic, short-term projects. Consultative forms of participation often take a one-size-fits-all approach, creating a single process and expecting the same form of contribution from all stakeholders. However, diverse stakeholders contribute differently and require different supports. Collaborative processes can better engage stakeholder perspectives by designing participation to be context and stakeholder specific, revisiting processes to ensure the appropriate information is given to and gathered from the appropriate stakeholders. 

\subsubsection{Unfilled seats}
Our co-design workshops represent a lower degree of participation along the dimension of stakeholder selection, as the included community members were chosen by the research team. According to Delgado et. al.'s framework, a participation process that truly empowers stakeholders involves engaging community members designated by the community itself. While valuable and necessary, this standard is difficult to achieve in the education context.

The education domain involves complex dynamic systems affected by the attributes of institutions, practitioners, communities and policy. While teachers contributed eagerly to the co-design of data specifications, participants across sessions grappled with the unknown perspectives of diverse domain-relevant stakeholders not represented in our workshops. Beyond students and teachers, groups named parents, district administrators, school counselors, instructional coaches, support staff and district personnel, community organizations, and policy makers as significant stakeholders in the design scenarios presented. Participants consistently demonstrated knowledge gaps regarding organizational structures in schools and school systems, struggling to identify data owners and match position titles to role-based responsibilities. While participants often referenced “administration” as an agentic entity and critical stakeholder, the specific practitioner role to call upon remains undefined. Further, teachers shared experiences in which they were required to perform the responsibilities of administration and support staff when those roles were unavailable. The complexity of education systems is exacerbated by constant organizational change, situational differences across individual institutions, and overlapping roles due to personnel turnover and resource strain. In the education domain, the non-trivial task of identifying the full set of appropriate stakeholders to bring to the table is a necessary precondition to multi-stakeholder collaboration.

\subsection{Scaffolding collaborative data specification}
Prior work in assessing engineering processes has noted the lack of defined practices for engaging domain experts and diverse stakeholders and the implications for the fairness and utility of the resulting systems \cite{subramonyam2021towards}. While we conducted workshops engaging participants in a structured data design task with guided questions, our findings demonstrate the need for additional scaffolding to support stakeholders in establishing common ground and continuous collaboration practices. 

\subsubsection{Initial groundwork}
Prior to the co-design workshops, participants were informed generally about the research motivations, but were not presented with the design scenario nor any information about data use in ML development until during the session. While this research design enabled us to observe practitioners navigating knowledge gaps, the introduction of initial groundwork may establish common ground and accelerate proactive contributions across participants. To help domain practitioners overcome technical knowledge gaps, collaborative processes require intentionally designed information scaffolds. While the lack of appropriate materials for educating domain experts on foundational ML knowledge is known ~\cite{bogina2022educating}, materials for educating ML practitioners on domain context are equally scarce. \mei{we just assume that it's the responsibility of non-technical experts to read up, but we don't make the same assumption about technical experts to learn about the domain} Pre-reading regarding the social and political context of the design scenario may seed a foundational understanding of domain needs, practices, and motivations. Further, participants reported feeling unsure about the quality of their contributions and uncertain about the expectations from their role. Establishing common ground and defining stakeholder roles prior to engaging in co-design may better prepare participants richer collaborative discussion. 

Initial groundwork may additionally define the collaborative context more effectively. Participants struggled with decision making due to a lack of clarity regarding the constraints of the design scenario. While the open-ended scenario invited high-level negotiations of priorities and requirements, groups reflected on the potential value of bounding ideation with real-world conditions, factoring financial, labor, and time resources into the initial formulation of the task. Finally, the inclusion of initial groundwork may enhance the generative design process, giving participants time to ideate independently before joint discussion and decision-making. 

\subsubsection{Shared standards}
Across sessions, groups struggled most with designing specifications for the evaluation of data quality. Participants found this task challenging due to the lack of shared language and metrics for data and system evaluation across disciplines. Non-technical stakeholders were unfamiliar with standard machine learning metrics, such as accuracy, prediction, and recall, and lacked context regarding their applied meanings for the given design scenario. Correspondingly, technical stakeholders were unable to translate practitioner calls for evaluations based on student learning outcomes into actionable data specifications. Despite recognizing the incompleteness of any existing metric, participants faced difficulties creating new ones that better serve contextual needs. We echo the call from prior work that fairness in ML requires the development of domain-specific metrics of quality \cite{shi2020artificial}.


%\mei{combat model-centric assumptions about data availability - scaffolding around feasibility assessment -- but also data ownership standards in the domain, who owns data should be known??}
%\mei{what does this mean for designers?? now that their roles were kind of taken over by this participatory pattern?}

\subsubsection{Continuous iteration}
According to Sloan et. al.'s framework, the most meaningful form of stakeholder involvement ("participation as justice") requires long-term partnerships with diverse stakeholders, building trust through mutual benefit, reciprocity, equity and tightly coupled relationships with frequent communication. To establish processes for cross-domain collaboration, prior work has highlighted the importance of design iteration with constant evaluation \cite{subramonyam2021towards}. 

Indeed, participants in every workshop session echoed this collaborative requirement, calling for stakeholder involvement at each step in the execution of the data specification. While domain practitioners appreciated the proactive data planning exercise, they expressed concerns about implementation fidelity and the potential for harmful assumptions to re-enter the development process in their absence. Some groups suggested the collaborative creation of a governing set of utility and ethical standards to be used in interval quality evaluations as new data decisions and trade-offs emerge. Involving multi-stakeholders in continuous collaboration requires the construction of a framework for iterative data specification, defining and scaffolding domain expert and end-user involvement in downstream data-decisions and evaluative data standards. While our findings illustrate the value of multi-stakeholder co-design of data specifications through a one-time collaboration, future work should explore the processes necessary to sustain iterative and long-term end-user and domain expert participation in data and machine learning development, in each stage of the data lifecycle and beyond.

\subsection{Limitations}
We present our data specification workshop procedure as a proof of concept with the acknowledgement that our sessions are subject to several limitations. Firstly, our sampling methods may have introduced selection bias, favoring stakeholders who felt fewer barriers to participation and displayed eagerness to seek collaborative work. Our participants additionally comprised an incomplete representation of stakeholders communities. Due to convenience and ethical regulations regarding participation in research, the student role was represented by undergraduate students, rather than younger students more accurately impacted by the largely K-12 design scenarios. We recruited ML engineers from a variety of research and industry backgrounds, and teachers specializing in various age groups and subject disciplines, and we do not account for the role of this heterogeneity in the participatory results.

Furthermore, our 2-hour workshop represents an oversimplified data specification process, 
The narrative surrounding the involvement of diverse stakeholders focuses on the prevention of harms by engaging domain context and impacted communities (e.g., \cite{boyarskaya2020overcoming}). Such framing, combined with latent structural inequality between stakeholder roles, limit the contribution of teachers to advocacy around well-recognized challenges in the education domain. When knowledge gaps are large enough, collaborative time is dedicated to establishing baseline domain understanding, leaving the the full potential of stakeholder contribution unexplored.
\mei{spell this out more, move it to limitations, longer or iterative sessions should be explored}

in which stakeholders interacted with the first author through prompts and guidance. These interactions may introduce a reactivity validity threat. Finally, the four design scenarios produced heterogeneity across sessions and introduced different challenges and design discussions due to the nature of the datasets involved (e.g., tabular, text, and image data). Some scenarios were more emotionally charged, while others were more challenging technically to stakeholders. For example, the undertone of surveillance in scenarios involving student images prompted richer discourse about racial biases, representation, and fairness than scenarios involving text data. While tabular data was easier to conceptualize, stakeholders were less familiar with image and text processing for data cleaning procedures, and these sessions relied heavily on technical experts to explain processing.

%\mei{Participatory AI project owners exert executive authority in deciding tactics of participation. AI researchers and practitioners feel caught between a desire to fulfill an idealized vision of empowered stakeholder participation and real-world constraint on time and resources.}







% The rapid development of machine learning (ML) applications in education has raised issues of fairness, accountability, transparency, and utility in their implications for practitioners and vulnerable student populations \cite{baker2022algorithmic, perrotta2020deep, pedro2019artificial}. Despite the promise of ML to facilitate learning processes with intelligent tools, ethical intentions are not by themselves sufficient \cite{holmes2022ethics, reich2017good}. The extensive adoption of ML applications in administration, instruction, and learning has been met with emerging ethical harms, including systematic inequalities in recommender systems \cite{marras2022equality} and high-stakes automated decision-making \cite{aied_chapter}, surveillance and civil rights concerns in facial recognition systems \cite{whittaker2018ai}, data privacy concerns \cite{potgieter2020privacy, feathers-1, feathers-2} and disparities in student propensities to consent \cite{li2022disparities}. The intensifying problem space is complicated by the underlying challenges facing ML in education: undefined policy-level guidelines \cite{schiff2022education}, insufficient teacher education and involvement in ML development \cite{bogina2022educating, schiff2021out, roll2016evolution}, underdevelopment of inclusive and high-quality data systems \cite{Ocumpaugh2014, gardner2019evaluating}, and lack of ethical regulation and transparency in data collection, use, and dissemination \cite{pedro2019artificial}. 

% One explanation behind unmet expectations of ML applications in education exists in the process tensions between engineering priorities and domain-specific practitioner needs. Traditional ML development processes undervalue the role of trustworthy training data and dataset accountability \cite{10.1145/3411764.3445518}. Despite the critical role of data in algorithmic predictions, training data is given inadequate consideration in current ML software workflows. Engineers often optimize the ML development process by defining data requirements -- including data types, features, labels, and the number of data points -- in an ad hoc manner. This approach falls short of capturing the needs of end-users and omits important contextual features of real-world data. While researchers have created guidelines for downstream data evaluation and documentation, standard practices remain undefined in upstream data specification.

% Furthermore, traditional engineering processes limit engagement with domain experts and end-users \cite{10.1145/3491102.3517537}. When included, diverse experts only converge in ML development after crucial data-related decisions have been made. Addressing the disconnects between stakeholders in development practices requires early collaboration, active construction of common ground, and co-created scaffolds to transcend knowledge boundaries. 

% As ML architectures stabilize, a recent methodological shift towards data-centric AI has re-prioritized the design of training data characteristics as the core mechanism to achieve desired performance. Data-centric methods present an opportunity to address fundamental data planning and collection issues by involving diverse stakeholders early in the ML development process.
\\
% We ask the following research questions: 
% \begin{itemize}
%     \item What do diverse stakeholders bring to the table when engaging in the proactive co-design of data specifications?
%     \item How can we systematically support and amplify diverse stakeholder voices in the ML data specification process?
% \end{itemize}


%\hari{What are our research questions? }

\begin{comment}
    


\hari{Positionality Statement, Threat to Validity}


\hari{What it takes to do the data work?}
\hari{Overcoming Blindness, Translation, Negotiation, Co-creation of Scaffolding}
\hari{Education Domain--- reach across boundaries through vulnerable first-person account, anecdotes, teach people technical, burden--- creating common ground}
\hari{Responsible Appropriate Use of data in Education}
\hari{data work, model work, application work is an engineering construct.... ``contextual data work''} 
\hari{Representation means so much and is very contextual (person + context) }


"Contextualizing ML Data Work In Education: Stakeholder Identities, Representations, and Common Ground/ Collaborative Practices/Desiderata for Collaboration" 


Contextualizing Data Needs/Work

Data Specifications for AI in Education: Representations, Identities, and Context / Contextualizing Data / Multi-Stakeholder Collaboration 

Data Specifications

Collaborative Data Needs/Specifications for AI in Education: Stakeholder Identities/ Translation Practices, Data Context 

A Seat at the table is not enough: Representation, 

Friction
Scaffolding Needs

Domain Experts have a lot to give in AI Specification in Education

Context, Translation, Identities 

multi-stakeholder collab
preemptive/proactive data spec
education focus

AI in Education

ML in Education: Data Specification, Multi-Stakeholder Identities, and Common Ground

A Seat at the Table: Multi-Stakeholder Data Specifications for AI in Education

Future Work: Shared language around ethics 

Data Needs for ML in Education: 

\end{comment}
